SydneyScapes: Image Segmentation for Australian Environments

Autonomous Vehicles (AVs) are being partially deployed and tested across various global locations, including China, the USA, Germany, France, Japan, Korea, and the UK, but with limited demonstrations in Australia. The integration of machine learning (ML) into AV perception systems highlights the need for locally labelled datasets to develop and test algorithms in specific environments. To address this, we introduce SydneyScapes - a dataset tailored for computer vision tasks of image semantic, instance, and panoptic segmentation. This dataset, collected from Sydney and surrounding cities in New South Wales (NSW), Australia, consists of 756 images with high-quality pixel-level annotations. It is designed to assist AV industry and researchers by providing annotated data and tools for algorithm development, testing, and deployment in the Australian context. Additionally, we offer benchmarking results using state-of-the-art algorithms to establish reference points for future research and development. The dataset is publicly available at https://hdl.handle.net/2123/33051.

==> backup/image_backup.tex <==
%Change this
\begin{figure}[h!]
\centering
\begin{subfigure}[]{0.48\columnwidth}
\centering
\includegraphics[width=\columnwidth]{ACRA2020_paper_Template/figures/nsw_dataset/frame-00000051-time-1649031915736001968.png}
\end{subfigure}
\begin{subfigure}[]{0.48\columnwidth}
\centering
\includegraphics[width=\columnwidth]{ACRA2020_paper_Template/figures/nsw_dataset/frame-00000426-time-1652076419027392864.png}
\end{subfigure}
\caption{\small Daytime image captures in different locations for the SydneyScapes dataset.}
\label{fig:NSW_dataset}
\end{figure}


%Change this
\begin{figure}[h!]
\centering
\begin{subfigure}[]{0.48\columnwidth}
\centering
\includegraphics[width=\columnwidth]{ACRA2020_paper_Template/figures/night_dataset/frame-00000036-time-1655885520669276953.png}
\end{subfigure}
\begin{subfigure}[]{0.48\columnwidth}
\centering
\includegraphics[width=\columnwidth]{ACRA2020_paper_Template/figures/night_dataset/frame-00000219-time-1655885902869277000.png}
\end{subfigure}

\caption{\small Nighttime images captures in different locations for the SydneyScapes dataset.}
\label{fig:NSW_dataset_night}
\end{figure}


%Change this
\begin{figure}[h!]
\centering
\begin{subfigure}[]{0.48\columnwidth}
\centering
\includegraphics[width=\columnwidth]{ACRA2020_paper_Template/figures/people_dataset/anonymous_frame-00005433-time-1667341429922091961.png}
\end{subfigure}
\begin{subfigure}[]{0.48\columnwidth}
\centering
\includegraphics[width=\columnwidth]{ACRA2020_paper_Template/figures/people_dataset/anonymous_frame-00006940-time-1660703309632294893.png}
\end{subfigure}
\caption{\small Images captures in different crowded locations for the SydneyScapes dataset.}
\label{fig:NSW_dataset_people}
\end{figure}



==> backup/table_backup.tex <==
\begin{table*}[htbp]
\centering
\caption{\textbf{Semantic segmentation results on SydneyScapes validation set}. * indicates that the method is trained on CityScapes \cite{Cordts2016Cityscapes}.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccccccccccccccc}
\toprule
\textbf{Category} & \multicolumn{2}{c}{\textbf{flat}} & \multicolumn{3}{c}{\textbf{construction}} & \multicolumn{3}{c}{\textbf{object}} & \multicolumn{2}{c}{\textbf{nature}} & \multicolumn{1}{c}{\textbf{sky}} & \multicolumn{2}{c}{\textbf{human}} & \multicolumn{6}{c}{\textbf{vehicle}} \\
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-6} \cmidrule(lr){7-9} \cmidrule(lr){10-11} \cmidrule(lr){12-12} \cmidrule(lr){13-14} \cmidrule(lr){15-20} \cmidrule(lr){21-21}
\textbf{Method} & \rotatebox{90}{\textbf{road}} & \rotatebox{90}{\textbf{sidewalk}} & \rotatebox{90}{\textbf{building}} & \rotatebox{90}{\textbf{wall}} & \rotatebox{90}{\textbf{fence}} & \rotatebox{90}{\textbf{pole}} & \rotatebox{90}{\textbf{traffic light}} & \rotatebox{90}{\textbf{traffic sign}} & \rotatebox{90}{\textbf{vegetation}} & \rotatebox{90}{\textbf{terrain}} & \rotatebox{90}{\textbf{sky}} & \rotatebox{90}{\textbf{person}} & \rotatebox{90}{\textbf{rider}} & \rotatebox{90}{\textbf{car}} & \rotatebox{90}{\textbf{truck}} & \rotatebox{90}{\textbf{bus}} & \rotatebox{90}{\textbf{train}} & \rotatebox{90}{\textbf{motorcycle}} & \rotatebox{90}{\textbf{bicycle}} & \rotatebox{90}{\textbf{mIoU}} \\
\midrule
BiSeNetV2* \cite{yu2021bisenet} & 73.84 & 45.43 & 72.49 & 1.86 & 23.92 & 26.84 & 25.24 & 28.78 & 66.92 & 41.96 & 82.5 & 60.37 & 32.13 & 48.56 & 31.87 & 40.45 & 5.99 & 20.58 & 34.45 &
40.22 \\ 
ISANet* \cite{huang2019interlaced} & 50.34 & 39.09 & 58.41 & 14.4 & 32.33 & 33.9 & 27.42 & 32.43 & 59.97 & 44.6 & 63.45 & 60.78 & 33.22 & 59.47 & 25.4 & 6.01 & 1.65 & 25.14 & 55.28 & 38.07 \\
STDC* \cite{fan2021rethinking} &  61.55 & 43.58 & 61.49 & 9.13 & 24.23 & 27.93 & 27.39 & 26.78 & 63.91 & 35.15 & 70.99 & 57.89 & 21.29 & 52.25 & 35.48 & 26.18 & 10.45 & 27.87 & 45.4 & 38.37 \\
SegFormer* \cite{xie2021segformer} & 80.76 & 49.9 & 75.21 & 2.73 & 32.11 & 39.21 & 47.07 & 35.53 & 73.12 & 58.93 & 86.42 & 70.83 & 43.59 & 69.0 & 48.66 & 26.34 & 2.82 & 32.01 & 56.4 & 48.98 \\
Mask2Former* \cite{cheng2022masked} & 88.16 & 57.02 & 79.39 & 2.02 & 24.47 & 39.01 & 43.9 & 42.99 & 73.48 & 53.15 & 88.39 & 75.29 & 43.02 & 80.86 & 61.03 & 52.92 & 2.95 & 59.31 & 68.87 & 54.54 \\
\midrule
BiSeNetV2 \cite{yu2021bisenet} & 93.49 & 72.55 & 85.72 & 46.05 & 47.44 & 36.27 & 45.35 & 31.08 & 82.6 & 80.61 & 96.86 & 60.88 & 0.0 & 81.24 & 55.98 & 53.17 & 0.0 & 40.47 & 3.74 & 53.34 \\ 
ISANet \cite{huang2019interlaced} & 95.56 & 79.62 & 90.3 & 59.42 & 65.97 & 51.07 & 70.01 & 63.47 & 87.46 & 84.54 & 97.47 & 76.14 & 34.45 & 89.72 & 74.17 & 78.02 & 0.0 & 43.38 & 57.18 & 68.31 \\ 
STDC \cite{fan2021rethinking} & 96.01 & 81.01 & 90.1 & 63.22 & 65.9 & 50.52 & 67.82 & 60.97 & 87.08 & 85.62 & 97.38 & 72.75 & 41.83 & 89.13 & 75.18 & 83.51 & 0.0 & 69.62 & 61.22 & 70.47 \\
SegFormer \cite{xie2021segformer} & 96.62 & 83.13 & 91.06 & 63.19 & 67.43 & 56.95 & 73.77 & 64.49 & 88.02 & 86.29 & 98.11 & 77.49 & 45.23 & 89.69 & 81.48 & 76.4 & 0.03 & 75.53 & 68.21 & 72.79 \\
Mask2Former \cite{cheng2022masked} & 97.3 & 87.03 & 92.58 & 60.27 & 74.97 & 70.7 & 81.88 & 72.22 & 89.77 & 88.7 & 98.3 & 83.04 & 55.04 & 92.93 & 84.05 & 86.12 & 2.18 & 80.23 & 69.8 & 77.21 \\
\bottomrule
\end{tabular}%
}
\end{table*}

\begin{table*}[htbp]
\centering
\caption{\textbf{Semantic segmentation results on SydneyScapes validation day subset}. * indicates that the method is trained on CityScapes \cite{Cordts2016Cityscapes}. - indicates that the field does not exist.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccccccccccccccc}
\toprule
\textbf{Category} & \multicolumn{2}{c}{\textbf{flat}} & \multicolumn{3}{c}{\textbf{construction}} & \multicolumn{3}{c}{\textbf{object}} & \multicolumn{2}{c}{\textbf{nature}} & \multicolumn{1}{c}{\textbf{sky}} & \multicolumn{2}{c}{\textbf{human}} & \multicolumn{6}{c}{\textbf{vehicle}} \\
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-6} \cmidrule(lr){7-9} \cmidrule(lr){10-11} \cmidrule(lr){12-12} \cmidrule(lr){13-14} \cmidrule(lr){15-20} \cmidrule(lr){21-21}
\textbf{Method} & \rotatebox{90}{\textbf{road}} & \rotatebox{90}{\textbf{sidewalk}} & \rotatebox{90}{\textbf{building}} & \rotatebox{90}{\textbf{wall}} & \rotatebox{90}{\textbf{fence}} & \rotatebox{90}{\textbf{pole}} & \rotatebox{90}{\textbf{traffic light}} & \rotatebox{90}{\textbf{traffic sign}} & \rotatebox{90}{\textbf{vegetation}} & \rotatebox{90}{\textbf{terrain}} & \rotatebox{90}{\textbf{sky}} & \rotatebox{90}{\textbf{person}} & \rotatebox{90}{\textbf{rider}} & \rotatebox{90}{\textbf{car}} & \rotatebox{90}{\textbf{truck}} & \rotatebox{90}{\textbf{bus}} & \rotatebox{90}{\textbf{train}} & \rotatebox{90}{\textbf{motorcycle}} & \rotatebox{90}{\textbf{bicycle}} & \rotatebox{90}{\textbf{mIoU}} \\
\midrule
BiSeNetV2* \cite{yu2021bisenet} & 65.92 & 27.82 & 66.41 & 3.7 & 20.89 & 16.04 & 14.66 & 25.95 & 70.84 & 46.68 & 85.98 & 10.8 & 0.0 & 28.63 & 7.33 & 42.64 & - & 45.04 & 0.0 & 32.19 \\ 
ISANet* \cite{huang2019interlaced} & 40.15 & 19.89 & 37.95 & 15.66 & 30.16 & 24.25 & 19.17 & 30.98 & 54.72 & 44.81 & 60.4 & 9.44 & 0.0 & 47.73 & 24.18 & 5.56 & - & 51.54 & 0.0 & 28.7 \\
STDC* \cite{fan2021rethinking} & 52.58 & 22.51 & 45.75 & 9.65 & 24.15 & 20.3 & 14.45 & 23.88 & 63.51 & 35.51 & 70.55 & 8.07 & 0.23 & 33.32 & 39.77 & 16.94 & - & 55.21 & 0.19 & 29.81 \\
SegFormer* \cite{xie2021segformer} & 77.7 & 41.09 & 65.12 & 3.03 & 30.85 & 30.82 & 28.44 & 40.04 & 75.35 & 61.11 & 90.81 & 26.7 & 0.0 & 56.14 & 35.3 & 16.49 & - & 55.84 & 2.0 & 40.94 \\
Mask2Former* \cite{cheng2022masked} & 85.1 & 40.93 & 72.92 & 1.81 & 23.08 & 23.33 & 22.41 & 40.72 & 74.47 & 60.08 & 92.2 & 26.42 & 0.0 & 71.87 & 57.92 & 62.51 & - & 74.44 & 0.0 & 46.12 \\
\midrule
BiSeNetV2 \cite{yu2021bisenet} & 93.54 & 65.97 & 80.71 & 54.13 & 48.09 & 30.11 & 20.95 & 29.3 & 86.09 & 81.41 & 98.33 & 36.82 & 0.0 & 70.4 & 52.17 & 70.67 & - & 58.95 & 0.0 & 54.31 \\ 
ISANet \cite{huang2019interlaced} & 94.96 & 70.63 & 86.48 & 69.04 & 68.61 & 42.71 & 48.43 & 66.72 & 89.35 & 85.79 & 98.6 & 57.54 & 5.73 & 83.21 & 73.43 & 77.62 & - & 59.48 & 0.0 & 65.46 \\ 
STDC \cite{fan2021rethinking} & 95.62 & 74.32 & 86.0 & 71.54 & 68.52 & 46.81 & 49.27 & 61.5 & 89.41 & 86.82 & 98.57 & 59.63 & 30.76 & 85.57 & 73.08 & 92.57 & - & 74.28 & 0.0 & 69.13 \\
SegFormer \cite{xie2021segformer} & 96.78 & 78.66 & 88.34 & 72.63 & 68.23 & 54.18 & 56.87 & 62.18 & 90.9 & 86.94 & 99.09 & 61.71 & 26.33 & 81.2 & 78.31 & 76.25 & - & 78.79 & 41.78 & 72.18 \\
Mask2Former \cite{cheng2022masked} & 97.39 & 83.2 & 88.93 & 72.35 & 72.42 & 67.56 & 72.82 & 63.48 & 91.74 & 89.14 & 99.1 & 67.79 & 44.35 & 87.59 & 79.42 & 97.64 & - & 85.23 & 0.0 & 75.56 \\
\bottomrule
\end{tabular}%
}
\end{table*}

\begin{table*}[htbp]
\centering
\caption{\textbf{Semantic segmentation results on SydneyScapes validation night subset}. * indicates that the method is trained on CityScapes \cite{Cordts2016Cityscapes}. - indicates that the field does not exist.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccccccccccccccc}
\toprule
\textbf{Category} & \multicolumn{2}{c}{\textbf{flat}} & \multicolumn{3}{c}{\textbf{construction}} & \multicolumn{3}{c}{\textbf{object}} & \multicolumn{2}{c}{\textbf{nature}} & \multicolumn{1}{c}{\textbf{sky}} & \multicolumn{2}{c}{\textbf{human}} & \multicolumn{6}{c}{\textbf{vehicle}} \\
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-6} \cmidrule(lr){7-9} \cmidrule(lr){10-11} \cmidrule(lr){12-12} \cmidrule(lr){13-14} \cmidrule(lr){15-20} \cmidrule(lr){21-21}
\textbf{Method} & \rotatebox{90}{\textbf{road}} & \rotatebox{90}{\textbf{sidewalk}} & \rotatebox{90}{\textbf{building}} & \rotatebox{90}{\textbf{wall}} & \rotatebox{90}{\textbf{fence}} & \rotatebox{90}{\textbf{pole}} & \rotatebox{90}{\textbf{traffic light}} & \rotatebox{90}{\textbf{traffic sign}} & \rotatebox{90}{\textbf{vegetation}} & \rotatebox{90}{\textbf{terrain}} & \rotatebox{90}{\textbf{sky}} & \rotatebox{90}{\textbf{person}} & \rotatebox{90}{\textbf{rider}} & \rotatebox{90}{\textbf{car}} & \rotatebox{90}{\textbf{truck}} & \rotatebox{90}{\textbf{bus}} & \rotatebox{90}{\textbf{train}} & \rotatebox{90}{\textbf{motorcycle}} & \rotatebox{90}{\textbf{bicycle}} & \rotatebox{90}{\textbf{mIoU}} \\
\midrule
BiSeNetV2* \cite{yu2021bisenet} & 48.36 & 21.68 & 43.26 & 0.0 & 0.0 & 9.54 & 1.75 & 21.12 & 51.77 & 0.12 & 14.76 & 15.79 & 22.71 & 24.22 & 0.0 & 0.0 & - & 0.0 & 25.14 & 16.68 \\ 
ISANet* \cite{huang2019interlaced} & 24.31 & 16.99 & 47.31 & 0.0 & 0.0 & 19.36 & 3.09 & 9.89 & 53.16 & 6.52 & 9.82 & 18.17 & 0.15 & 20.29 & 0.0 & 0.0 & - & 7.42 & 55.12 & 16.2 \\
STDC* \cite{fan2021rethinking} & 27.41 & 22.02 & 40.97 & 0.0 & 0.0 & 12.96 & 2.19 & 12.05 & 51.32 & 3.08 & 8.36 & 18.9 & 0.0 & 21.15 & 0.0 & 0.0 & - & 5.46 & 32.81 & 14.37 \\
SegFormer* \cite{xie2021segformer} & 65.59 & 23.6 & 54.7 & 0.0 & 0.0 & 20.25 & 30.99 & 19.23 & 57.98 & 0.84 & 13.62 & 20.73 & 27.93 & 45.98 & 0.0 & 0.0 & - & 14.36 & 45.19 & 24.5 \\
Mask2Former* \cite{cheng2022masked} & 81.53 & 34.14 & 59.53 & 0.0 & 0.05 & 27.17 & 8.07 & 36.82 & 62.47 & 0.19 & 24.16 & 41.94 & 45.65 & 64.67 & 1.92 & 0.0 & - & 50.18 & 77.56 & 34.23 \\
\midrule
BiSeNetV2 \cite{yu2021bisenet} & 92.27 & 69.98 & 80.89 & 0.0 & 0.0 & 26.73 & 29.39 & 32.42 & 75.28 & 0.0 & 85.42 & 18.73 & 0.0 & 79.63 & 0.0 & 0.0 & - & 44.55 & 0.0 & 35.29 \\ 
ISANet \cite{huang2019interlaced} & 95.46 & 76.1 & 85.62 & 0.0 & 23.8 & 36.93 & 43.74 & 64.48 & 81.53 & 0.74 & 89.21 & 46.03 & 51.24 & 87.66 & 14.76 & 0.0 & - & 31.72 & 40.4 & 48.30 \\ 
STDC \cite{fan2021rethinking} & 95.62 & 77.69 & 85.6 & 0.0 & 12.23 & 35.5 & 39.78 & 54.95 & 80.64 & 1.83 & 88.48 & 52.26 & 37.62 & 88.41 & 8.21 & 0.0 & - & 70.92 & 67.64 & 52.62 \\
SegFormer \cite{xie2021segformer} & 95.01 & 76.01 & 84.9 & 0.0 & 4.99 & 33.02 & 46.7 & 56.68 & 79.82 & 5.94 & 89.23 & 45.19 & 39.71 & 87.2 & 9.65 & 0.0 & - & 77.43 & 65.62 & 49.84 \\
Mask2Former \cite{cheng2022masked} & 96.7 & 84.27 & 88.02 & 0.0 & 69.68 & 56.19 & 52.53 & 68.61 & 83.27 & 0.0 & 91.07 & 53.47 & 66.63 & 90.97 & 12.36 & 0.0 & - & 78.6 & 43.41 & 57.54 \\
\bottomrule
\end{tabular}%
}
\end{table*}

\begin{table*}[htbp]
\centering
\caption{\textbf{Semantic segmentation results on SydneyScapes validation people subset}. * indicates that the method is trained on CityScapes \cite{Cordts2016Cityscapes}.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccccccccccccccc}
\toprule
\textbf{Category} & \multicolumn{2}{c}{\textbf{flat}} & \multicolumn{3}{c}{\textbf{construction}} & \multicolumn{3}{c}{\textbf{object}} & \multicolumn{2}{c}{\textbf{nature}} & \multicolumn{1}{c}{\textbf{sky}} & \multicolumn{2}{c}{\textbf{human}} & \multicolumn{6}{c}{\textbf{vehicle}} \\
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-6} \cmidrule(lr){7-9} \cmidrule(lr){10-11} \cmidrule(lr){12-12} \cmidrule(lr){13-14} \cmidrule(lr){15-20} \cmidrule(lr){21-21}
\textbf{Method} & \rotatebox{90}{\textbf{road}} & \rotatebox{90}{\textbf{sidewalk}} & \rotatebox{90}{\textbf{building}} & \rotatebox{90}{\textbf{wall}} & \rotatebox{90}{\textbf{fence}} & \rotatebox{90}{\textbf{pole}} & \rotatebox{90}{\textbf{traffic light}} & \rotatebox{90}{\textbf{traffic sign}} & \rotatebox{90}{\textbf{vegetation}} & \rotatebox{90}{\textbf{terrain}} & \rotatebox{90}{\textbf{sky}} & \rotatebox{90}{\textbf{person}} & \rotatebox{90}{\textbf{rider}} & \rotatebox{90}{\textbf{car}} & \rotatebox{90}{\textbf{truck}} & \rotatebox{90}{\textbf{bus}} & \rotatebox{90}{\textbf{train}} & \rotatebox{90}{\textbf{motorcycle}} & \rotatebox{90}{\textbf{bicycle}} & \rotatebox{90}{\textbf{mIoU}} \\
\midrule
BiSeNetV2* \cite{yu2021bisenet} & 90.29 & 67.12 & 85.78 & 9.29 & 37.78 & 36.36 & 29.25 & 31.64 & 76.77 & 21.36 & 91.19 & 67.31 & 36.67 & 80.02 & 55.91 & 46.72 & 6.81 & 20.03 & 52.32 & 49.61 \\ 
ISANet* \cite{huang2019interlaced} & 70.55 & 56.52 & 75.72 & 9.44 & 40.13 & 41.11 & 31.03 & 37.27 & 77.82 & 37.62 & 86.18 & 67.63 & 39.27 & 82.32 & 30.56 & 27.73 & 3.03 & 8.65 & 57.14 & 46.30 \\
STDC* \cite{fan2021rethinking} & 82.84 & 65.84 & 80.14 & 7.45 & 25.12 & 35.7 & 31.86 & 30.82 & 77.34 & 27.09 & 88.9 & 65.4 & 34.73 & 78.07 & 32.19 & 45.65 & 24.11 & 5.23 & 59.24 & 47.25 \\
SegFormer* \cite{xie2021segformer} & 89.0 & 63.43 & 88.64 & 5.22 & 42.04 & 46.75 & 51.98 & 36.52 & 81.87 & 33.78 & 93.94 & 74.05 & 47.36 & 85.39 & 63.77 & 41.5 & 10.07 & 15.44 & 63.04 & 54.41 \\
Mask2Former* \cite{cheng2022masked} & 93.78 & 76.95 & 89.93 & 3.37 & 44.53 & 50.73 & 51.36 & 45.25 & 80.65 & 22.96 & 95.25 & 78.82 & 46.16 & 91.3 & 69.78 & 48.05 & 9.51 & 26.06 & 67.79 & 57.48 \\
\midrule
BiSeNetV2 \cite{yu2021bisenet} & 93.79 & 77.03 & 89.08 & 0.46 & 46.6 & 41.47 & 50.88 & 31.68 & 82.35 & 36.91 & 96.07 & 63.02 & 0.0 & 86.68 & 60.99 & 43.83 & 0.0 & 0.1 & 4.41 & 47.65 \\ 
ISANet \cite{huang2019interlaced} & 96.28 & 85.94 & 93.16 & 10.12 & 61.31 & 58.76 & 76.3 & 61.74 & 88.71 & 58.66 & 96.67 & 77.71 & 32.65 & 93.2 & 76.52 & 78.29 & 0.0 & 28.91 & 66.48 & 65.34 \\ 
STDC \cite{fan2021rethinking} & 96.58 & 85.73 & 93.02 & 25.35 & 61.49 & 56.11 & 73.57 & 61.92 & 88.04 & 45.35 & 96.59 & 73.62 & 42.75 & 90.87 & 78.9 & 78.42 & 0.0 & 21.17 & 60.23 & 64.72 \\
SegFormer \cite{xie2021segformer} & 96.91 & 87.81 & 94.01 & 16.84 & 66.67 & 64.43 & 79.46 & 67.24 & 89.54 & 55.11 & 97.92 & 78.81 & 46.49 & 94.23 & 86.53 & 76.56 & 0.03 & 22.64 & 68.87 & 67.90 \\
Mask2Former \cite{cheng2022masked} & 97.37 & 89.98 & 95.35 & 8.02 & 80.41 & 76.11 & 86.34 & 78.19 & 91.3 & 71.22 & 98.09 & 84.58 & 52.75 & 95.92 & 90.53 & 80.18 & 2.18 & 39.13 & 79.21 & 73.52 \\
\bottomrule
\end{tabular}%
}
\end{table*}

==> backup/table_backup2.tex <==
\begin{table*}[h]
\centering
\caption{\textbf{Semantic segmentation results on the SydneyScapes validation set and its subsets}. \raisebox{0pt}[0pt][0pt]{\colorbox{lightblue}{Blue}} represents results for the day subset (first and second sections). \raisebox{0pt}[0pt][0pt]{\colorbox{lightyellow}{Yellow}} represents results for the night subset (third and fourth sections). \raisebox{0pt}[0pt][0pt]{\colorbox{lightgray}{Gray}} represents results for the people subset (fifth and sixth sections). \raisebox{0pt}[0pt][0pt]{\colorbox{lightgreen}{Green}} represents results for the full validation set (seventh and eighth sections). The methods evaluated are ISANet \cite{huang2019interlaced}, BiSeNetV2 \cite{yu2021bisenet}, STDC \cite{fan2021rethinking}, SegFormer \cite{xie2021segformer}, and Mask2Former \cite{cheng2022masked}. An asterisk (*) denotes methods trained on CityScapes \cite{Cordts2016Cityscapes}. A hyphen (-) indicates that the field is not applicable.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccccccccccccccc}
\toprule
\textbf{Group} & \multicolumn{3}{c}{\textbf{flat}} & \multicolumn{3}{c}{\textbf{construction}} & \multicolumn{3}{c}{\textbf{object}} & \multicolumn{2}{c}{\textbf{nature}} & \multicolumn{2}{c}{\textbf{human}} & \multicolumn{6}{c}{\textbf{vehicle}} \\
\cmidrule(lr){1-1} \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14} \cmidrule(lr){15-20} \cmidrule(lr){21-21}
\textbf{Method} & \rotatebox{90}{\textbf{road}} & \rotatebox{90}{\textbf{sidewalk}} & \rotatebox{90}{\textbf{terrain}} & \rotatebox{90}{\textbf{building}} & \rotatebox{90}{\textbf{wall}} & \rotatebox{90}{\textbf{fence}} & \rotatebox{90}{\textbf{pole}} & \rotatebox{90}{\textbf{traffic light}} & \rotatebox{90}{\textbf{traffic sign}} & \rotatebox{90}{\textbf{vegetation}} & \rotatebox{90}{\textbf{sky}} & \rotatebox{90}{\textbf{person}} & \rotatebox{90}{\textbf{rider}} & \rotatebox{90}{\textbf{car}} & \rotatebox{90}{\textbf{truck}} & \rotatebox{90}{\textbf{bus}} & \rotatebox{90}{\textbf{on rails}} & \rotatebox{90}{\textbf{motorcycle}} & \rotatebox{90}{\textbf{bicycle}} & \rotatebox{90}{\textbf{mIoU}} \\
\midrule
\rowcolor{lightblue} BiSeNetV2* \cite{yu2021bisenet} & 65.92 & 27.82 & 46.68 & 66.41 & 3.7 & 20.89 & 16.04 & 14.66 & 25.95 & 70.84 & 85.98 & 10.8 & 0.0 & 28.63 & 7.33 & 42.64 & - & 45.04 & 0.0 & 32.19 \\ 
\rowcolor{lightblue} ISANet* \cite{huang2019interlaced} & 40.15 & 19.89 & 44.81 & 37.95 & 15.66 & 30.16 & 24.25 & 19.17 & 30.98 & 54.72 & 60.4 & 9.44 & 0.0 & 47.73 & 24.18 & 5.56 & - & 51.54 & 0.0 & 28.7 \\
\rowcolor{lightblue} STDC* \cite{fan2021rethinking} & 52.58 & 22.51 & 35.51 & 45.75 & 9.65 & 24.15 & 20.3 & 14.45 & 23.88 & 63.51 & 70.55 & 8.07 & 0.23 & 33.32 & 39.77 & 16.94 & - & 55.21 & 0.19 & 29.81 \\
\rowcolor{lightblue} SegFormer* \cite{xie2021segformer} & 77.7 & 41.09 & 61.11 & 65.12 & 3.03 & 30.85 & 30.82 & 28.44 & 40.04 & 75.35 & 90.81 & 26.7 & 0.0 & 56.14 & 35.3 & 16.49 & - & 55.84 & 2.0 & 40.94 \\
\rowcolor{lightblue} Mask2Former* \cite{cheng2022masked} & 85.1 & 40.93 & 60.08 & 72.92 & 1.81 & 23.08 & 23.33 & 22.41 & 40.72 & 74.47 & 92.2 & 26.42 & 0.0 & 71.87 & 57.92 & 62.51 & - & 74.44 & 0.0 & 46.12 \\
\midrule
\rowcolor{lightblue} BiSeNetV2 \cite{yu2021bisenet} & 93.54 & 65.97 & 81.41 & 80.71 & 54.13 & 48.09 & 30.11 & 20.95 & 29.3 & 86.09 & 98.33 & 36.82 & 0.0 & 70.4 & 52.17 & 70.67 & - & 58.95 & 0.0 & 54.31 \\ 
\rowcolor{lightblue} ISANet \cite{huang2019interlaced} & 94.96 & 70.63 & 85.79 & 86.48 & 69.04 & 68.61 & 42.71 & 48.43 & 66.72 & 89.35 & 98.6 & 57.54 & 5.73 & 83.21 & 73.43 & 77.62 & - & 59.48 & 0.0 & 65.46 \\ 
\rowcolor{lightblue} STDC \cite{fan2021rethinking} & 95.62 & 74.32 & 86.82 & 86.0 & 71.54 & 68.52 & 46.81 & 49.27 & 61.5 & 89.41 & 98.57 & 59.63 & 30.76 & 85.57 & 73.08 & 92.57 & - & 74.28 & 0.0 & 69.13 \\
\rowcolor{lightblue} SegFormer \cite{xie2021segformer} & 96.78 & 78.66 & 86.94 & 88.34 & 72.63 & 68.23 & 54.18 & 56.87 & 62.18 & 90.9 & 99.09 & 61.71 & 26.33 & 81.2 & 78.31 & 76.25 & - & 78.79 & 41.78 & 72.18 \\
\rowcolor{lightblue} Mask2Former \cite{cheng2022masked} & 97.39 & 83.2 & 89.14 & 88.93 & 72.35 & 72.42 & 67.56 & 72.82 & 63.48 & 91.74 & 99.1 & 67.79 & 44.35 & 87.59 & 79.42 & 97.64 & - & 85.23 & 0.0 & 75.56 \\
\midrule
\rowcolor{lightyellow} BiSeNetV2* \cite{yu2021bisenet} & 48.36 & 21.68 & 0.12 & 43.26 & 0.0 & 0.0 & 9.54 & 1.75 & 21.12 & 51.77 & 14.76 & 15.79 & 22.71 & 24.22 & 0.0 & 0.0 & - & 0.0 & 25.14 & 16.68 \\ 
\rowcolor{lightyellow} ISANet* \cite{huang2019interlaced} & 24.31 & 16.99 & 6.52 & 47.31 & 0.0 & 0.0 & 19.36 & 3.09 & 9.89 & 53.16 & 9.82 & 18.17 & 0.15 & 20.29 & 0.0 & 0.0 & - & 7.42 & 55.12 & 16.2 \\
\rowcolor{lightyellow} STDC* \cite{fan2021rethinking} & 27.41 & 22.02 & 3.08 & 40.97 & 0.0 & 0.0 & 12.96 & 2.19 & 12.05 & 51.32 & 8.36 & 18.9 & 0.0 & 21.15 & 0.0 & 0.0 & - & 5.46 & 32.81 & 14.37 \\
\rowcolor{lightyellow} SegFormer* \cite{xie2021segformer} & 65.59 & 23.6 & 0.84 & 54.7 & 0.0 & 0.0 & 20.25 & 30.99 & 19.23 & 57.98 & 13.62 & 20.73 & 27.93 & 45.98 & 0.0 & 0.0 & - & 14.36 & 45.19 & 24.5 \\
\rowcolor{lightyellow} Mask2Former* \cite{cheng2022masked} & 81.53 & 34.14 & 0.19 & 59.53 & 0.0 & 0.05 & 27.17 & 8.07 & 36.82 & 62.47 & 24.16 & 41.94 & 45.65 & 64.67 & 1.92 & 0.0 & - & 50.18 & 77.56 & 34.23 \\
\midrule
\rowcolor{lightyellow} BiSeNetV2 \cite{yu2021bisenet} & 92.27 & 69.98 & 0.0 & 80.89 & 0.0 & 0.0 & 26.73 & 29.39 & 32.42 & 75.28 & 85.42 & 18.73 & 0.0 & 79.63 & 0.0 & 0.0 & - & 44.55 & 0.0 & 35.29 \\ 
\rowcolor{lightyellow} ISANet \cite{huang2019interlaced} & 95.46 & 76.1 & 0.74 & 85.62 & 0.0 & 23.8 & 36.93 & 43.74 & 64.48 & 81.53 & 89.21 & 46.03 & 51.24 & 87.66 & 14.76 & 0.0 & - & 31.72 & 40.4 & 48.30 \\ 
\rowcolor{lightyellow} STDC \cite{fan2021rethinking} & 95.62 & 77.69 & 1.83 & 85.6 & 0.0 & 12.23 & 35.5 & 39.78 & 54.95 & 80.64 & 88.48 & 52.26 & 37.62 & 88.41 & 8.21 & 0.0 & - & 70.92 & 67.64 & 52.62 \\
\rowcolor{lightyellow} SegFormer \cite{xie2021segformer} & 95.01 & 76.01 & 5.94 & 84.9 & 0.0 & 4.99 & 33.02 & 46.7 & 56.68 & 79.82 & 89.23 & 45.19 & 39.71 & 87.2 & 9.65 & 0.0 & - & 77.43 & 65.62 & 49.84 \\
\rowcolor{lightyellow} Mask2Former \cite{cheng2022masked} & 96.7 & 84.27 & 0.0 & 88.02 & 0.0 & 69.68 & 56.19 & 52.53 & 68.61 & 83.27 & 91.07 & 53.47 & 66.63 & 90.97 & 12.36 & 0.0 & - & 78.6 & 43.41 & 57.54 \\
\midrule
\rowcolor{lightgray} BiSeNetV2* \cite{yu2021bisenet} & 90.29 & 67.12 & 21.36 & 85.78 & 9.29 & 37.78 & 36.36 & 29.25 & 31.64 & 76.77 & 91.19 & 67.31 & 36.67 & 80.02 & 55.91 & 46.72 & 6.81 & 20.03 & 52.32 & 49.61 \\ 
\rowcolor{lightgray} ISANet* \cite{huang2019interlaced} & 70.55 & 56.52 & 37.62 & 75.72 & 9.44 & 40.13 & 41.11 & 31.03 & 37.27 & 77.82 & 86.18 & 67.63 & 39.27 & 82.32 & 30.56 & 27.73 & 3.03 & 8.65 & 57.14 & 46.30 \\
\rowcolor{lightgray} STDC* \cite{fan2021rethinking} & 82.84 & 65.84 & 27.09 & 80.14 & 7.45 & 25.12 & 35.7 & 31.86 & 30.82 & 77.34 & 88.9 & 65.4 & 34.73 & 78.07 & 32.19 & 45.65 & 24.11 & 5.23 & 59.24 & 47.25 \\
\rowcolor{lightgray} SegFormer* \cite{xie2021segformer} & 89.0 & 63.43 & 33.78 & 88.64 & 5.22 & 42.04 & 46.75 & 51.98 & 36.52 & 81.87 & 93.94 & 74.05 & 47.36 & 85.39 & 63.77 & 41.5 & 10.07 & 15.44 & 63.04 & 54.41 \\
\rowcolor{lightgray} Mask2Former* \cite{cheng2022masked} & 93.78 & 76.95 & 22.96 & 89.93 & 3.37 & 44.53 & 50.73 & 51.36 & 45.25 & 80.65 & 95.25 & 78.82 & 46.16 & 91.3 & 69.78 & 48.05 & 9.51 & 26.06 & 67.79 & 57.48 \\
\midrule
\rowcolor{lightgray} BiSeNetV2 \cite{yu2021bisenet} & 93.79 & 77.03 & 36.91 & 89.08 & 0.46 & 46.6 & 41.47 & 50.88 & 31.68 & 82.35 & 96.07 & 63.02 & 0.0 & 86.68 & 60.99 & 43.83 & 0.0 & 0.1 & 4.41 & 47.65 \\ 
\rowcolor{lightgray} ISANet \cite{huang2019interlaced} & 96.28 & 85.94 & 58.66 & 93.16 & 10.12 & 61.31 & 58.76 & 76.3 & 61.74 & 88.71 & 96.67 & 77.71 & 32.65 & 93.2 & 76.52 & 78.29 & 0.0 & 28.91 & 66.48 & 65.34 \\ 
\rowcolor{lightgray} STDC \cite{fan2021rethinking} & 96.58 & 85.73 & 45.35 & 93.02 & 25.35 & 61.49 & 56.11 & 73.57 & 61.92 & 88.04 & 96.59 & 73.62 & 42.75 & 90.87 & 78.9 & 78.42 & 0.0 & 21.17 & 60.23 & 64.72 \\
\rowcolor{lightgray} SegFormer \cite{xie2021segformer} & 96.91 & 87.81 & 55.11 & 94.01 & 16.84 & 66.67 & 64.43 & 79.46 & 67.24 & 89.54 & 97.92 & 78.81 & 46.49 & 94.23 & 86.53 & 76.56 & 0.03 & 22.64 & 68.87 & 67.90 \\
\rowcolor{lightgray} Mask2Former \cite{cheng2022masked} & 97.37 & 89.98 & 71.22 & 95.35 & 8.02 & 80.41 & 76.11 & 86.34 & 78.19 & 91.3 & 98.09 & 84.58 & 52.75 & 95.92 & 90.53 & 80.18 & 2.18 & 39.13 & 79.21 & 73.52 \\
\midrule
\rowcolor{lightgreen} BiSeNetV2* \cite{yu2021bisenet} & 73.84 & 45.43 & 41.96 & 72.49 & 1.86 & 23.92 & 26.84 & 25.24 & 28.78 & 66.92 & 82.5 & 60.37 & 32.13 & 48.56 & 31.87 & 40.45 & 5.99 & 20.58 & 34.45 & 40.22 \\ 
\rowcolor{lightgreen} ISANet* \cite{huang2019interlaced} & 50.34 & 39.09 & 44.6 & 58.41 & 14.4 & 32.33 & 33.9 & 27.42 & 32.43 & 59.97 & 63.45 & 60.78 & 33.22 & 59.47 & 25.4 & 6.01 & 1.65 & 25.14 & 55.28 & 38.07 \\
\rowcolor{lightgreen} STDC* \cite{fan2021rethinking} &  61.55 & 43.58 & 35.15 & 61.49 & 9.13 & 24.23 & 27.93 & 27.39 & 26.78 & 63.91 & 70.99 & 57.89 & 21.29 & 52.25 & 35.48 & 26.18 & 10.45 & 27.87 & 45.4 & 38.37 \\
\rowcolor{lightgreen} SegFormer* \cite{xie2021segformer} & 80.76 & 49.9 & 58.93 & 75.21 & 2.73 & 32.11 & 39.21 & 47.07 & 35.53 & 73.12 & 86.42 & 70.83 & 43.59 & 69.0 & 48.66 & 26.34 & 2.82 & 32.01 & 56.4 & 48.98 \\
\rowcolor{lightgreen} Mask2Former* \cite{cheng2022masked} & 88.16 & 57.02 & 53.15 & 79.39 & 2.02 & 24.47 & 39.01 & 43.9 & 42.99 & 73.48 & 88.39 & 75.29 & 43.02 & 80.86 & 61.03 & 52.92 & 2.95 & 59.31 & 68.87 & 54.54 \\
\midrule
\rowcolor{lightgreen} BiSeNetV2 \cite{yu2021bisenet} & 93.49 & 72.55 & 80.61 & 85.72 & 46.05 & 47.44 & 36.27 & 45.35 & 31.08 & 82.6 & 96.86 & 60.88 & 0.0 & 81.24 & 55.98 & 53.17 & 0.0 & 40.47 & 3.74 & 53.34 \\ 
\rowcolor{lightgreen} ISANet \cite{huang2019interlaced} & 95.56 & 79.62 & 84.54 & 90.3 & 59.42 & 65.97 & 51.07 & 70.01 & 63.47 & 87.46 & 97.47 & 76.14 & 34.45 & 89.72 & 74.17 & 78.02 & 0.0 & 43.38 & 57.18 & 68.31 \\ 
\rowcolor{lightgreen} STDC \cite{fan2021rethinking} & 96.01 & 81.01 & 85.62 & 90.1 & 63.22 & 65.9 & 50.52 & 67.82 & 60.97 & 87.08 & 97.38 & 72.75 & 41.83 & 89.13 & 75.18 & 83.51 & 0.0 & 69.62 & 61.22 & 70.47 \\
\rowcolor{lightgreen} SegFormer \cite{xie2021segformer} & 96.62 & 83.13 & 86.29 & 91.06 & 63.19 & 67.43 & 56.95 & 73.77 & 64.49 & 88.02 & 98.11 & 77.49 & 45.23 & 89.69 & 81.48 & 76.4 & 0.03 & 75.53 & 68.21 & 72.79 \\
\rowcolor{lightgreen} Mask2Former \cite{cheng2022masked} & 97.3 & 87.03 & 88.7 & 92.58 & 60.27 & 74.97 & 70.7 & 81.88 & 72.22 & 89.77 & 98.3 & 83.04 & 55.04 & 92.93 & 84.05 & 86.12 & 2.18 & 80.23 & 69.8 & 77.21 \\
\bottomrule
\end{tabular}%
}
\end{table*}


\begin{table*}[h]
\centering
\caption{\textbf{Instance segmentation results on the SydneyScapes validation set and its subsets}. \raisebox{0pt}[0pt][0pt]{\colorbox{lightblue}{Blue}} represents results for the day subset (first and second sections). \raisebox{0pt}[0pt][0pt]{\colorbox{lightyellow}{Yellow}} represents results for the night subset (third and fourth sections). \raisebox{0pt}[0pt][0pt]{\colorbox{lightgray}{Gray}} represents results for the people subset (fifth and sixth sections). \raisebox{0pt}[0pt][0pt]{\colorbox{lightgreen}{Green}} represents results for the full validation set (seventh and eighth sections). The methods evaluated are Mask R-CNN \cite{he2017mask}, PointRend \cite{kirillov2020pointrend}, and Mask2Former \cite{cheng2022masked}. An asterisk (*) denotes methods trained on CityScapes \cite{Cordts2016Cityscapes}. A hyphen (-) indicates that the field is not applicable.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccccccc}
\toprule
\textbf{Group} & \multicolumn{2}{c}{\textbf{human}} & \multicolumn{6}{c}{\textbf{vehicle}} \\
\cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-9}
\textbf{Method} & \rotatebox{90}{\textbf{person}} & \rotatebox{90}{\textbf{rider}} & \rotatebox{90}{\textbf{car}} & \rotatebox{90}{\textbf{truck}} & \rotatebox{90}{\textbf{bus}} & \rotatebox{90}{\textbf{on rails}} & \rotatebox{90}{\textbf{motorcycle}} & \rotatebox{90}{\textbf{bicycle}} & \rotatebox{90}{\textbf{AP}} & \rotatebox{90}{\textbf{$\text{AP}_\text{50}$}} \\
\midrule
\rowcolor{lightblue} PointRend* \cite{kirillov2020pointrend} & 20.3 & 0.0 & 23.6 & 4.0 & 5.6 & - & 4.3 & 0.0 & 8.3 & 16.3 \\
\rowcolor{lightblue} Mask2Former* \cite{cheng2022masked} & 33.2 & 0.3 & 32.9 & 4.6 & 4.6 & - & 26.3 & 3.7 & 15.1 & 27.4 \\
\rowcolor{lightblue} Mask R-CNN* \cite{he2017mask} &  23.4 & 0.0 & 31.1 & 10.0 & 25.0 & - & 25.0 & 0.0 & 16.4 & 27.1 \\
\midrule
\rowcolor{lightblue} PointRend \cite{kirillov2020pointrend} & 34.9 & 0.0 & 45.2 & 25.0 & 25.0 & - & 19.5 & 0.0 & 21.4 & 37.6 \\
\rowcolor{lightblue} Mask2Former \cite{cheng2022masked} & 36.2 & 0.0 & 44.1 & 20.2 & 15.0 & - & 30.2 & 40.0 & 26.5 & 50.2 \\
\rowcolor{lightblue} Mask R-CNN \cite{he2017mask} &  32.4 & 0.0 & 43.5 & 21.8 & 25.0 & - & 24.6 & 0.0 & 21.0 & 33.5 \\
\midrule
\rowcolor{lightyellow} PointRend* \cite{kirillov2020pointrend} & 7.0 & 11.9 & 6.4 & 0.0 & - & - & 0.0 & 20.0 & 7.5 & 21.8 \\
\rowcolor{lightyellow} Mask2Former* \cite{cheng2022masked} & 13.2 & 27.5 & 22.9 & 0.0 & - & - & 0.1 & 37.8 & 16.9 & 35.1 \\
\rowcolor{lightyellow} Mask R-CNN* \cite{he2017mask} & 11.3 & 12.5 & 12.1 & 0.0 & - & - & 6.0 & 47.4 & 14.9 & 30.1 \\
\midrule
\rowcolor{lightyellow} PointRend \cite{kirillov2020pointrend} & 22.3 & 27.5 & 47.0 & 0.0 & - & - & 26.0 & 33.3 & 26.0 & 44.3 \\
\rowcolor{lightyellow} Mask2Former \cite{cheng2022masked} & 25.4 & 25.6 & 46.3 & 25.0 & - & - & 30.3 & 53.3 & 34.3 & 64.5 \\
\rowcolor{lightyellow} Mask R-CNN \cite{he2017mask} &  24.3 & 25.6 & 46.6 & 7.5 & - & - & 17.1 & 60.6 & 30.3 & 60.8 \\
\midrule
\rowcolor{lightgray} PointRend* \cite{kirillov2020pointrend} & 26.7 & 19.2 & 39.4 & 15.2 & 18.3 & 0.0 & 1.5 & 11.7 & 16.5 & 31.0 \\
\rowcolor{lightgray} Mask2Former* \cite{cheng2022masked} & 32.8 & 11.6 & 40.1 & 10.4 & 15.9 & 0.0 & 11.7 & 17.1 & 17.5 & 33.5 \\
\rowcolor{lightgray} Mask R-CNN* \cite{he2017mask} & 32.9 & 22.0 & 39.7 & 16.4 & 20.0 & 4.2 & 3.6 & 15.3 & 19.3 & 35.7 \\
\midrule
\rowcolor{lightgray} PointRend \cite{kirillov2020pointrend} & 35.9 & 20.0 & 46.2 & 26.0 & 35.5 & 0.0 & 11.5 & 17.0 & 24.0 & 45.7 \\
\rowcolor{lightgray} Mask2Former \cite{cheng2022masked} & 31.3 & 22.6 & 43.0 & 32.1 & 37.5 & 0.0 & 9.9 & 16.8 & 24.1 & 45.1 \\
\rowcolor{lightgray} Mask R-CNN \cite{he2017mask} & 37.2 & 18.6 & 45.4 & 28.0 & 43.4 & 0.0 & 13.2 & 17.3 & 25.4 & 46.9 \\
\midrule
\rowcolor{lightgreen} PointRend* \cite{kirillov2020pointrend} & 26.1 & 15.1 & 29.1 & 9.4 & 17.1 & 0.0 & 2.1 & 11.3 & 13.8 & 27.0 \\
\rowcolor{lightgreen} Mask2Former* \cite{cheng2022masked} & 32.5 & 12.2 & 35.2 & 7.1 & 14.1 & 0.0 & 13.0 & 18.0 & 16.5 & 31.7 \\
\rowcolor{lightgreen} Mask R-CNN* \cite{he2017mask} & 32.2 & 18.3 & 32.6 & 12.1 & 20.4 & 4.2 & 12.3 & 16.3 & 18.6 & 35.5 \\
\midrule
\rowcolor{lightgreen} PointRend \cite{kirillov2020pointrend} & 35.6 & 19.2 & 45.9 & 24.5 & 34.6 & 0.0 & 15.4 & 17.7 & 24.1 & 45.0 \\
\rowcolor{lightgreen} Mask2Former \cite{cheng2022masked} & 31.2 & 21.2 & 43.8 & 26.9 & 35.3 & 0.0 & 17.5 & 19.4 & 24.4 & 45.8 \\
\rowcolor{lightgreen} Mask R-CNN \cite{he2017mask} &  36.8 & 17.9 & 44.8 & 23.4 & 41.6 & 0.0 & 17.7 & 20.3 & 25.3 & 45.8 \\
\bottomrule
\end{tabular}%
}
\end{table*}
